Learning Model Preconditions for Planning with Multiple Models

Different models can provide differing levels of fidelity when a robot is planning. Analytical models are often fast to evaluate but only work in limited ranges of conditions. Meanwhile, physics simulators are effective at modeling complex interactions between objects but are typically more computationally expensive. Learning when to switch between the various models can greatly improve the speed of planning and task success reliability. In this work, we learn model deviation estimators (MDEs) to predict the error between real-world states and the states outputted by transition models. MDEs can be used to define a model precondition that describes which transitions are accurately modeled. We then propose a planner that uses the learned model preconditions to switch between various models in order to use models in conditions where they are accurate, prioritizing faster models when possible. We evaluate our method on two real-world tasks: placing a rod into a box and placing a rod into a closed drawer.

==> corl_sections/result_old_mde_eval.tex <==
 A grid was adding to the x and y values of the rod locations and the robot.  Hyperparameter optimization for KNN, GPR, and RFR were done using $L_g$ as a scoring function. The MLP was directly optimized on $L_g$. Hyperparameter grid search values and more details about data augmentation are available in Appendix~\ref{mdetrainingdetails}.


We evaluate the MDEs' precision and recall for several different MDE representations: k-nearest neighbors (KNN), Gaussian Processes (GPR), Random Forests (RFR), linear regression, and a multi-layer perceptron (MLP). We use scikit-learn~\citep{scikit-learn} implementations except for the MLP, and hyperparameter optimize using 4-fold cross validation for 20 iterations. Details about hyperparameter ranges and other implementation details are in Appendix~\ref{mdetrainingdetails}
At a threshold of 7 cm, the most practical for \texttt{RodInBox}, the model with the best performance was the MLP, likely because the loss function is directly optimized rather than used for hyperparameter optimization. Though the precision for the MDE implemented with an MLP was lower than for KNN, RFR, and GPR, the recall was much higher, which reflects our objective where deviation underestimates are worse than overestimates. Only results for $\textit{LiftAndDrop}$ are shown for brevity, as it is the most complex skill to learn $\hat{d}$ for since $d(s_t,a_t, \theta_t)$ relies on small differences in $s_t$ and $\theta_t$. For the rest of the results, we use an MLP as the MDE representation as it demonstrated the best performance. 

    \begin{figure}
        \centering
        \includegraphics[width=\textwidth]{imgs/precision_recall.pdf}
        \caption{Precision and recall for deviation models}
        \label{fig:precisionrecall}
        \vspace{-0.2cm}
    \end{figure}
        


%         \begin{figure}
%             \centering
%             \includegraphics[width=\textwidth]{imgs/sample_complexity.pdf}
%             \caption{Sample complexity analysis . We show $L_g$ over the number of training samples}
%             \label{fig:samplecomplexity}
%         \end{figure}

% In Figure ~\ref{fig:samplecomplexity} we show $L_g$ for different numbers of training samples, randomly subsampled from the training set to measure sample complexity for the different models. 




==> corl_sections/suboptimality_bound_old_mha.tex <==
% \documentclass{article}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% \usepackage{todonotes}
% \newtheorem{theorem}{Theorem}[]
% \newtheorem{lemma}[theorem]{Lemma}
% \begin{document}
%Justify the intuition behind the weights
%\newcommand{\open}{\text{open}}
%\newcommand{\closed}{\text{closed}}
\newcommand{\minw}{\mathrm{min}(w)}
\newcommand{\wtwo}{\frac{w_1}{\minw}}
%\newcommand{\sbest}{s}
%\newcommand{\citep}[1]{ \textit{Citation placeholder} }
%\renewcommand{\cite}[1]{ \textit{Citation placeholder} }

Next, we show guaranteed suboptimality bounds for using our algorithm using both PS and PE under some additional assumptions. The main transformation is that we only consider edges executing $a$ from $s$ to reach $s'$ if it can be accurately modelled by at least one $M$. Otherwise, the edge does not exist. The guarantees are only on the plan; our method for learning $\mathrm{pre}(M)$ using MDEs does not have formal guarantees on the state of the system. 

\textbf{Assumptions: }
\begin{itemize}
    \item \textbf{Optional if we don't guarantee termination}: There is at least one path to $s_g$ using $(s,a) \in \bigcup \mathrm{pre}(M)$. 
    \item $M_i(s,a) = M_j(s,a) \forall (i,j) s.t. (s,a) \in \mathrm{pre}(M_i) \cap \mathrm{pre}(M_j)$, we know that all models will predict the same discrete state if correct. 
    \item $\epsilon > 1$
    \item $w_i >= w_j$ if $i < j$, reflecting decreasing penalty for each model
    \item $h$ is admissible and consistent
    \item $c(s,s') \geq 0$
    \item If $(s,a)$ is not in $\mathrm{pre}(M)$ for any $M$ in the problem, any outgoing edge using $a$ from $s$ has infinite cost
\end{itemize}


\begin{theorem} If MRA* with PS terminates, $g(s_g) \leq \epsilon g^*(s_g)$ \end{theorem}
\begin{proof}
Since the rule for expansion in PS is to select $\mathrm{max}_i s.t. s,a \in \mathrm{pre}(M_i)$, if $ s,a \in \bigcup \mathrm{pre}(M_i)$, then there will be at least model that can be used to compute $s'$. Otherwise, that edge does not exist. Because of Assumption 2, successors for any $s$ is the same whether computed using $M_i$ or $M_j$. Thus, if $\exists M s.t. (s,a) \in \mathrm{pre}(M)$, $s'$ will be computed. Since $c(s,a,s')$ is not dependent on $M$, the cost will be the same, so $g(s')$ is not dependent on the model. Therefore, using PS does not change the properties of WA*. 

Using the fact that MRA* with PS is a special case of WA*, the cost to $s_g$ found using MRA* using PS is upper bounded by $\epsilon g^*(s_g)$. The bound follows from the proof in ~\citep{likhachev2003ara}. 
\end{proof}

\begin{theorem}{If MRA* with PE terminates, $g(s_g) \leq \frac{w_0}{\minw}\epsilon g^*(s_g)$} \end{theorem}
\begin{proof}
Here, we show that $g(s_g) \leq \frac{w_1}{\minw} g^*(s_g)$ when using MRA with PE by showing it is a special case of MHA*. Shared MHA* uses $K$ different heuristics and separate priority queues for each heuristic. MHA* makes use of an \textit{anchor} search, which is the only search that must use an admissible heuristic. We show how the selection rule to decide between full expansion and partial expansion in PE is equivalent to using the anchor search and inadmissible search in MHA*. Then we show how full expansion is a case of anchor search, and that the partial expansions can be considered the additional searches for MHA*.  

Our search when $i=0$ is equivalent to the anchor search in MHA* because it uses an admissible and consistent heuristic. MHA* does not require admissibility or consistency from the other heuristics. The weighting factor used to inflate the heuristic value in our algorithm is $\epsilon \geq 1.0$, which is a constant, just like in~\citep{likhachev2003ara}.  

According to Equation~\ref{eq:rewrittenpe}, if $\open_i.MinKey() \geq \wtwo \open_0.MinKey()$, then $\sbest$ from $\open_0$ is expanded and placed in $\closed_0$. Since that means all possible actions have been evaluated and $h$ is the same for all searches, we place it in all other $\closed$ as well. 

Searches for $i=1$ can be considered special cases of inadmissible searches in MHA. The proof for suboptimality for MHA* does not \textit{require} the heuristics be inadmissible.
If $\open_i.MinKey() \leq \wtwo \open_0.MinKey()$ where $i>0$, then $\sbest$ from $\open_i$ is expanded, and added to $\closed_i$ just like in MHA*. The set of possible successors from $s$ using $\bigcup M s.t. (s,a) \in \mathrm{pre}(M)$ is a superset of the possible successors that can be computed using any one model, because $M \subseteq \bigcup M$. Thus, it is not possible to compute an edge by expanding from $\open_i$ that cannot be expanded using $\open_0$. Therefore, expanding from any $\open_i$ for $i > 0$ using prioritized expansion has the same properties as using the inadmissible queues for speedup in MHA*. 

Finally, we show that the parameters used to select between models can be written as the parameters used to select between searches in MHA*. The relevant hyperparameters for computing a suboptimality guarantee for MRA* with PE are $w_0$ and $\minw$. $\minw$ is equal to the final element $w_{K-1}$ because $w_i < w_j$ if $i > j$. 

Using Equation~\ref{eq:expansionrule}, the anchor search is selected when the following condition holds: 
\begin{equation}
%Write the same way as it would be in MHA*
\wtwo \open_0 MinKey () \leq OPEN_i.MinKey() \forall i > 0
\label{eq:rewrittenpe}
\end{equation} 



Thus, $\wtwo$ is the variable used to prioritize inadmissible searches over the anchor search. The proof in ~\cite{aine2016multi} for suboptimality of MHA* does not use the fact that nodes from the inadmissible queues are expanded in a round-robin manner. Therefore, we can use the result that $g(s) \leq \alpha g^*(s) \forall s$ for some constant $\alpha$ to guarantee that $g(s_g) \leq \alpha g^*(s_g)$ where $\alpha = \wtwo$.

%Although all elements in $w$ should generally reflect preference between using one model over another based on computational cost, the only weights that affect the suboptimality bound are $w_0$ and $\minw$, 

\end{proof}

%\end{document}

==> plan_example_utils/sAsB.tex <==
            \node<3-4> (sA) [planNodeSmall, right of=s0, xshift=\nodespacing, sASty] {$s_a$};
            \node<3-4> [gLabel,below=0.0 cm of sA]{\scriptsize $g=1$};
            \node<3-4> (sB) [planNodeSmall, right of=sA, xshift=\nodespacing, sBSty] {$s_b$};
            \node<3-4> [gLabel,below=0.0 cm of sB]{\scriptsize $g=1$};

==> plan_example_utils/sAsBpersist.tex <==
            \node<3-> (sA) [planNodeSmall, right of=s0, xshift=\nodespacing, sASty] {$s_a$};
            \node<3-> [gLabel,below=0.0 cm of sA]{\scriptsize $g=1$};
            \node<3-> (sB) [planNodeSmall, right of=sA, xshift=\nodespacing, sBSty] {$s_b$};
            \node<3-> [gLabel,below=0.0 cm of sB]{\scriptsize $g=1$};
